Layer-wise Linear Mode Connectivity

Averaging neural network parameters is an intuitive method for fusing the knowledge of two independent models. It is most prominently used in federated learning. If models are averaged at the end of training, this can only lead to a good performing model if the loss surface of interest is very particular, i.e., the loss in the midpoint between the two models needs to be sufficiently low. This is impossible to guarantee for the non-convex losses of state-of-the-art networks. For averaging models trained on vastly different datasets, it was proposed to average only the parameters of particular layers or combinations of layers, resulting in better performing models. To get a better understanding of the effect of layer-wise averaging, we analyse the performance of the models that result from averaging single layers, or groups of layers. Based on our empirical and theoretical investigation, we introduce a novel notion of the layer-wise linear connectivity, and show that deep networks do not have layer-wise barriers between them.

==> setup.tex <==
\section{Setup}
\label{apx:sec:setup}

In order to discuss the results in a more structured and formal way several definitions have to be explained in detail.
In particular, which models are we averaging, how does it reflect in the loss surface understanding and what does it say about the models similarity.



Some of the minima are reparametrizations of each other and then they can be made linearly connected by perturbations.
With it they might or might not be connected by a non-linear path.
So non-linear path creates valleys of minima, linear connectivity convex basins and perturbations are for putting minima in one or another basin.

\subsection{What parameter configurations do we consider?}
Usually linear connectivity is assumed to exist for trained networks, since they should be positioned in the same basin on the loss surface.
Nevertheless, even the parameters of trained networks are almost never exact (mathematically) critical points.
As it was pointed out, what we are finding with SGD is not a local optimum, but a direction in which the loss surface is very flat~\footnote{(c) Andrew G. Wilson in his talk for \href{https://www.epfl.ch/labs/lcn/epfl-virtual-symposium-loss-landscape-of-neural-networks-theoretical-insights-and-practical-implications-15-16-february-2022/}{EPFL workshop on loss surfaces}.\TODO{MA: can we cite his paper instead? otherwise, we reveal a bit our identity.}}.
The works on feature matching usually assume for their setup some trained networks~\citep{garipov2018loss, draxler2018essentially, singh2020model, jordan2022repair}.
On the other hand, in the federated learning averaging is performed throughout the training and without any expectation that the averaged model lies in the same basin as current local models.
Thus, we consider neural networks that were trained for some number of epochs and perform good on the training set, i.e., lie in the region of low (more or less) training loss.
%Let's call such neural networks \textbf{solutions}.

\subsection{Basin of solutions}
%It is usually assumed that some kind of low-loss basins exists in the loss surface of DNNs.
While different equal loss basins are explained by reparametrizations of solutions, thus assuming that functionally they are equivalent, differences of the models within one basin are less intuitive.
On the one hand, they are capable of producing a performant ensembles~\citep{wortsman2022model} and thus should be functionally different.
On the other hand, they are claimed to be similar in the terms of linear connectivity~\citep{entezarirole}.
Even more controversial is the opinion that solutions from different basins are necessary for a good performing ensemble~\citep{fort2019deep}.
It is not clear if the assumption of the existence of such basins also includes the assumption of them being convex.
Nevertheless, from previous research~\citep{garipov2018loss, draxler2018essentially} it is known that they do not have to be convex---they can have an arbitrary shape and points in them can be connected by a non-linear path of low loss value.
In this research we are approaching the federated setup from the loss surface perspective, therefore we need to consider exactly convex basins allowing for successful averaging.

\subsection{Similarity of neural networks}
There exist different techniques to estimate the similarity of two neural networks. 
%For example the cosine similarity between parameters allows to measure the distance of two networks in the parameter space.
However, since the dimensionality of the parameter space of nowadays neural networks is enormously high, using standard distance measures for understanding their similarity is questionable.
Moreover, equioutput reparametrizations~\citep{petzka2020notes} make it impossible to define closeness of the models just through the closeness  of points in the parameter space.
Measuring the closeness in function space is challenging as well.
Most definitely, having the same training loss does not imply that networks are the same.
Having the same training as well as testing loss can hint that the performance of the networks is similar.
Analysing the similarity in the per sample prediction can give an even better indication of functional similarity - in general all the "correct" models should be functionally similar to the function underlying the data generation process (if it is uniquely defined by the training data given).
In particular, the linear connectivity can also be considered as similarity measure between two models, which will have the additional meaning in the federated setup as an indicator of successful averaging.
Such similarity not only indicates the loss similarity, but also implicitly describes the loss surface surrounding the models.
It is important to notice, that barriers between configurations can be measured in terms of loss or in terms of prediction error.
From our perspective, while the test error is a better indicator for final performance, the loss is more significant for understanding the loss surface---since it is loss values that guide the dynamic of the training.
